Signatures From Pseudorandom States via $\bot$-PRFs

Different flavors of quantum pseudorandomness have proven useful for various cryptographic applications, with the compelling feature that these primitives are potentially weaker than post-quantum one-way functions. Ananth, Lin, and Yuen (2023) have shown that logarithmic pseudorandom states can be used to construct a pseudo-deterministic PRG: informally, for a fixed seed, the output is the same with $1-1/poly$ probability. In this work, we introduce new definitions for $\bot$-PRG and $\bot$-PRF. The correctness guarantees are that, for a fixed seed, except with negligible probability, the output is either the same (with probability $1-1/poly$) or recognizable abort, denoted $\bot$. Our approach admits a natural definition of multi-time PRG security, as well as the adaptive security of a PRF. We construct a $\bot$-PRG from any pseudo-deterministic PRG and, from that, a $\bot$-PRF. Even though most mini-crypt primitives, such as symmetric key encryption, commitments, MAC, and length-restricted one-time digital signatures, have been shown based on various quantum pseudorandomness assumptions, digital signatures remained elusive. Our main application is a (quantum) digital signature scheme with classical public keys and signatures, thereby addressing a previously unresolved question posed in Morimae and Yamakawa's work (Crypto, 2022). Additionally, we construct CPA secure public-key encryption with tamper-resilient quantum public keys.

==> QPKE.tex <==
\section{Tamper-Proof Quantum Public-Key Encryption From PD-PRG}

The main result of this section is as follows.

\begin{theorem}\label{thm:qpke-from-pdprf}
    Assuming the existence of a  ($\mu,\ell)$-$\botPRG$ for some inverse polynomial $\mu(\secpar)$. for some $\mu(\secpar)$ satisfying $\mu(\secpar)\cdot\secpar\in \poly$, there exists a $\cpatamp$ secure $\QPKE$ scheme (as defined in~\cite{KMNY23}).
\end{theorem}

\begin{proof}[Sketch]
We prove the theorem in the following steps.
\begin{enumerate}
    \item First, we show that instantiating the construction in~\cite{KMNY23} with a $(1-\delta(\lambda))$-correct digital signature scheme for some inverse polynomial function $\delta()$, produces a $(1-\delta(\lambda))$-correct $\QPKE$ scheme $\Pi$ which is $\cpatamp$ secure. By \Cref{lemma:cor-digital-sig,thm:sec sig}, we know that exists a $(1-\delta(\lambda))$-correct digital signature scheme based on $\PDPRF$, for some  inverse polynomial function $\delta(\lambda)$. For more details, see \Cref{thm:qpke-from-pdprf-restated-imperfect-correctness} in \Cref{subsec:construct-qpke-proof}.
    \item Next, we do a variant of $\lambda$ parallel repetition of $\Pi$ to get a $\QPKE$ scheme $\Pi^\lambda$ that satisfies negligible correctness error.  We also show that this $\lambda$-fold $\QPKE$ scheme is also $\cpatamp$ secure since the original scheme was $\cpatamp$ secure. For more details, see \Cref{thm:qpke-parallel-repetition-lift} in \Cref{subsec:construct-qpke-proof}. \qed
\end{enumerate}

\end{proof}

The full proof is given in \Cref{subsec:construct-qpke-proof}.

% The construction is the same as in~\cite{KMN23}, but we instantiate the construction with a $(1-\delta(\lambda))$-correct digital signature scheme for some inverse polynomial function $\delta()$. Note that by \Cref{lemma:cor-digital-sig,thm:sec sig} \anote{add reference}, such a digital signature scheme can be based on bot-PRFs. It is easy to verify that the resulting scheme is at least as secure as the scheme in~\cite{KMN23}, because the correctness error means that the challenger sometimes sends $\bot$ to the adversary in the CPA game, which can only harm the success probability of the adversary. However, note that the encryption scheme will be $(1-\delta(\lambda))$ correct. Next, we do parallel repetition to boost the correctness error to negligible. Finally, we conclude the security of the parallel repeated scheme by showing that if a tamper-proof quantum encryption scheme satisfies CPA security, then any $r(\lambda)$ times parallel repeated version of it is also CPA secure, as long as $r(\lambda)\in \poly[\lambda]$.


==> appx-DS.tex <==
\section{Correct Digital Signatures}
\label{sec:corr sig}
The correctness error of our DS scheme (Construction \ref{con:many-time sig}) can be improved to allow for negligible error by simple repetition, as we show in the following construction. 

\begin{construct}
\label{con:correct sig}
Let $\lambda\in \mathbb{N}$ be the security parameter and let $\overline{\Pi}\coloneqq (\overline{\textsf{KeyGen}},\overline{\textsf{Sign}},\overline{\textsf{Verify}})$ be the algorithms of a SUF DS scheme on $n$-bit messages with $(1/p)$-correctness, where $p\in {\poly[\lambda]}$. The algorithms for a correct DS scheme on $n$-bit messages is as follows:
\begin{itemize}
    \item $\textsf{KeyGen}(1^\lambda):$ 
    \begin{enumerate}
        \item For each $i\in [3p]$, sample $(\textsf{sk}_i,\textsf{vk}_i)\leftarrow \overline{\textsf{Gen}}(1^\lambda)$. 
        \item Set $\sk \coloneqq (\sk_i)_{i\in [3p]}$ and $\vk \coloneqq (\vk_i)_{i\in [3p]}$.
        \item Output $(\sk,\vk)$.
    \end{enumerate}

    \item $\textsf{Sign}(\sk,m):$ 
    \begin{enumerate}
        \item For each $i\in [3p],$ compute $\sigma_i\leftarrow \overline{\textsf{Sign}}(\sk_i,m).$
        \item If $\sigma_i=\perp$ for all $i\in [3p]$, then output $\perp$.
        \item Otherwise, let $\sigma_j$ be the first non $\perp$ signature. Output $(j,\sigma_j).$
    \end{enumerate}

  
     \item $\textsf{Verify}(\vk,m,\sigma):$ 
     \begin{enumerate}
         \item If $\sigma =\perp$, then output $\perp$. 
         \item Otherwise, parse $\sigma$ as $(j,\sigma_j)$.
         \item Output $\overline{\textsf{Verify}}(\vk_j,m,\sigma_j)$.
     \end{enumerate}
  
\end{itemize}
\end{construct}


\begin{theorem}
\label{thm:corr sig}
Construction \ref{con:correct sig} is a correct and SUF DS scheme assuming the existence of a SUF $(1/p)$-correct DS scheme. 
\end{theorem}

\begin{proof}
    It is clear that there is a negligible chance that the signature of a message is $\perp$ by the $(1/p)$-correctness property of $\overline{\Pi}$

    For security, assume for contradiction that there exists a QPT adversary $\adv$ which breaks SUF of the scheme. We construct an adversary $\overline{\adv}$ which breaks the SUF of $\overline{\Pi}$. 

    In the SUF experiment $\textsf{Sign}^{\text{SUF}}_{\overline{\Pi}, \overline{\adv}}({\lambda})$, the experiment first samples a key pair $(\overline{\sk},\overline{\vk})\leftarrow \overline{\textsf{KeyGen}}(1^\lambda)$. $\overline{\adv}$ receives $\overline{\vk}$ and oracle access to $\overline{\textsf{Sign}}(\overline{\sk},\cdot)$. The algorithm for $\overline{\adv}$ is as follows:
    \begin{enumerate}
        \item $\overline{\adv}$ randomly picks $j\leftarrow [3p]$.
        \item For each $i\in [3p]/j$, $\overline{\adv}$ samples $(\sk_i,\vk_i)\leftarrow \overline{\textsf{KeyGen}}(1^\lambda)$.
        \item $\overline{\adv}$ sets $\vk_j\coloneqq \overline{\vk}$ and ${\vk}\coloneqq (\vk_i)_{i\in [3p]}$. 
        \item $\overline{\adv}$ runs $\adv({\vk})$ and answers signature queries by $\adv$ using oracle access to $\overline{\textsf{Sign}}(\sk,\cdot)$ as well as the signing keys $(\sk_i)_{i\in [3p]/j}$ as described in $\textsf{Sign}$.
  \item Let $\mathcal{Q}$ denote the set of messages-signature pairs returned by the signing oracle.        
  \item $\adv$ outputs forgery $(m^*,(k,\sigma^*_k))$. 
   \item If $k=j$, then $\overline{\adv}$ outputs $(m^*,(k,\sigma^*_k))$ and outputs $\perp$ otherwise. 
   \end{enumerate}  

By our assumption, there is a non-negligible probability that $\adv$ outputs a forgery not in $\mathcal{Q}$. In this case, there is $\frac{1}{3p}$ probability that $j=k$ since $j$ is indistinguishable from random with respect to $\adv$. Hence, with non-negligible probability $\adv$ forges a new signature under $\tilde{\vk}$ breaking the SUF of $\overline{\Pi}$.   
    \qed
\end{proof}


==> garbage.tex <==
\section{Pseudo-Deterministic One-Way and Universal One-Way Hash Functions} 

We introduce the notion of \emph{pseudo-deterministic one-way functions} (PD-OWF) and show how to construct them from $\SPRS$s. PD-OWF will then be used in \cref{sec:qpduowhfsect} to construct pseudo-deterministic universal one-way hash function families allowing Rompel's procedure to transform Lamport's one-time scheme into a many-time stateful one \cite{R90}.

\subsection{Pseudo-Deterministic One-Way Functions}\label{sec:def_owf}

We define pseudo-deterministic one-way functions similarly to the pseudo-deterministic pseudo-random generators (Def.~\ref{def:PD-PRG}).

%\subsection{Definition}
\begin{definition}[Pseudo-deterministic One-Way Functions]
\label{def:PD-OWF}
    A QPT function $F:\{0,1\}^{m(\lambda)}\rightarrow \{0,1\}^{\ell(\lambda)}$, where $m(\cdot)$ and $\ell(\cdot)$ are polynomials, is a \emph{pseudo-deterministic one-way function (PD-OWF)} when the following conditions hold:
    \begin{itemize}   
        \item (Pseudo-determinism) There exists constant $c>0$ and function $\mu(\lambda)\in O(\lambda^{-c})$ such that for all $\lambda\in \mathbb{N}$, there exists a set $\mathcal{K}_\lambda \subset \{0,1\}^{m(\lambda)}$:
        \begin{enumerate}
            \item $\Pr[x\in \mathcal{K}_\lambda:x\leftarrow \{0,1\}^{m(\lambda)}]\geq 1-{\mu(\lambda)}.$
            \item For any $x\in \mathcal{K}_\lambda$:
            \[
                \max_{y\in \{0,1\}^{\ell(\lambda)}}\Pr[y=F(x)]\geq 1-{\mu(\lambda)} .
            \]
        \end{enumerate}
        \item (Security) For every QPT inverter $\adv$:
        \begin{align*}
             \Pr_{x\leftarrow \{0,1\}^{m(\lambda)}}[F(\adv(F(x)))=F(x)]\leq \negl[\lambda] .
        \end{align*}
    \end{itemize}
    A pseudo-deterministic function with non-determinism function $\mu$ is denoted as \emph{$\mu(\lambda)$-PD-OWF}. 
\end{definition}

\subsubsection{Construction.}
We show that PD-OWFs can be built from $\SPRS$s. Recall $\PDPRG$s (Definition \ref{def:PD-PRG}) were constructed from $\SPRS$s (Lemma \ref{lem:PD-PRG}). We convert the PD-PRG into a PD-OWF to obtain the following result:

\begin{theorem}
    \label{thm:OWF}
 Assuming the existence of $(c\log \lambda)$-PRS with $c>12$, there exists a $O(\lambda^{-c/12+1})$-PD-OWF $F:\{0,1\}^{\ell(\lambda)}\rightarrow \{0,1\}^{\ell(\lambda)}$ with input/output length $\ell(\lambda)=\lambda^{c/6}$.
   \end{theorem}

\begin{proof}
    By Lemma \ref{lem:PD-PRG}, $(c\log \lambda)$-PRS with $c>12$ implies the existence of a $O(\lambda^{-c/12+1})$-PD-PRG $G:\{0,1\}^{\lambda^2}\rightarrow \{0,1\}^{\ell(\lambda)}$. Define the function $F: \{0,1\}^{\ell(\lambda)}\rightarrow \{0,1\}^{\ell(\lambda)}$ by $F(z)=F(x,y)\coloneqq G(x)$ where the input $z\in \{0,1\}^{\ell(\lambda)}$ is parsed into $x\in \{0,1\}^{\lambda^2} $ and $y\in \{0,1\}^{\ell(\lambda)-\lambda^2}$. It is clear that $F$ satisfies the pseudo-determinism condition for PD-OWFs (Definition \ref{def:PD-OWF}). We claim that $F$ also satisfies the security condition. 

    Assume this is not true, then there exists a QPT algorithm $\adv$ and polynomial $p(\cdot)\geq 0$ such that:
    \begin{align*}
        \Pr_{z\leftarrow \{0,1\}^{\ell(\lambda)}}[F(\adv(F(z)))=F(z)]\geq \frac{1}{p(\lambda)}.
    \end{align*}
This is equivalent to:
    \begin{align*}
        \Pr_{x\leftarrow \{0,1\}^{\lambda^2}}[G(\adv(G(x)))=G(x)]\geq \frac{1}{p(\lambda)}.
    \end{align*}
Now, construct a QPT algorithm $\adv'$ which can distinguish outputs of $G$ from random.  

    \begin{construct} \textbf{Algorithm} $\adv'(y)$:
        \begin{enumerate}
            \item Run $\adv(y)$ and let $x'$ be the result. 
            \item If $G(x')=y$ then output 1 and output 0 otherwise. 
        \end{enumerate}
    \end{construct}

Define the set of deterministic images of $G$ as $\mathcal{Y}_\lambda \coloneqq \{y: \ \exists x \in \{0,1\}^{\lambda^2}| \ \Pr[G(x)=y]\geq \frac{1}{2^\lambda}\}$. Each element of the input can map to at most $2^\lambda$ elements in $\mathcal{Y}_\lambda$ so $|\mathcal{Y}_\lambda |\leq 2^{\lambda^2+\lambda}$. This means $\Pr_{y\leftarrow \{0,1\}^{\ell(\lambda)}}[y\in \mathcal{Y}_\lambda]\leq \negl[\lambda]$. 

Now sample $y\leftarrow \{0,1\}^{\ell(\lambda)}$, then the probability any value $x$ maps to $y$ is given by:
\begin{align*}
    \Pr[G(x)=y]=\Pr[(G(x)=y) \wedge (y\in \mathcal{Y}_\lambda) ] +\Pr[(G(x)=y) \wedge ( y\notin \mathcal{Y}_\lambda) ]\leq \negl[\lambda],
\end{align*}
where $\Pr[(G(x)=y) \wedge ( y\notin \mathcal{Y}_\lambda) ]\leq 2^{-\lambda}$ by definition of $\mathcal{Y}_\lambda$. 
Hence, the probability that $\Pr_{y\leftarrow \{0,1\}^{\ell(\lambda)}}[\adv'(y)=1]\leq \negl[\lambda]$.

Meanwhile, for a value sampled from the image of $G$, we have:
\begin{align*}
    \Pr_{x\leftarrow \{0,1\}^\lambda}[\adv'(G(x))=1]=\Pr_{x\leftarrow \{0,1\}^{\lambda}}[G(\adv(G(x)))=G(x)]\geq \frac{1}{p(\lambda)} .
\end{align*}
In other words, $\adv'$ can distinguish the output of $G$ from random which gives a contradiction. Hence, $F$ satisfies the security condition of PD-OWFs. 
\qed
\end{proof}

\subsection{Pseudo-Deterministic Universal One-Way Hash Functions}
\label{sec:qpduowhfsect}

We define the notion of pseudo-deterministic universal one-way hash function families as the natural non-deterministic version of universal one-way hash functions (Def.~\ref{def:uowhf}). Building universal one-way hash function families from any one-way function
was Rompel's main contribution allowing to conclude that one-way functions are sufficient for
many-time stateful signatures\cite{R90}. 
%\subsection{Definition}
%We define the notion of PD-UOWHFs as they will be used in our signature scheme. 

\begin{definition}[PD-UOWHF]
    A class $\mathcal{H}:\{0,1\}^{m(\lambda)}\rightarrow \{0,1\}^{\ell(\lambda)}$, where $m(\cdot)$ and $\ell(\cdot)$ are polynomials, is a family of QPT \emph{PD-UOWHFs} if it satisfies the following three properties:
    \begin{enumerate}
            \item (Pseudo-determinism) There exists constant $c>0$ and function $\mu(\lambda)=O(\lambda^{-c})$ such that for any $F\in \mathcal{H}$ and $\lambda\in \mathbb{N}$, there exists a set $\mathcal{K}_{m} \subset \{0,1\}^{m(\lambda)}$ such that:
        \begin{enumerate}
            \item $\Pr[x\in \mathcal{K}_{m}:x\leftarrow \{0,1\}^{m(\lambda)}]\geq 1-\mu(\lambda).$
            \item For any $x\in \mathcal{K}_{m}$:
            \begin{align*}
                \max_{y\in \{0,1\}^{\ell(\lambda)}}\Pr[y=F(x)]\geq 1-\mu(\lambda).
            \end{align*}
            where the probability is taken over the randomness of $F$.
        \end{enumerate}
        \item (One-wayness) For any $F\in \mathcal{H}$ and QPT inverter $\adv$:
        \begin{align*}
             \Pr_{x\leftarrow \{0,1\}^m}[F(\adv(F(x)))=F(x)]\leq \negl[\lambda].
        \end{align*}

        \item (Collision-resistance) For every QPT algorithm $\adv$, if $\adv$ outputs $x$ and then is given $F\leftarrow \mathcal{H}$, then the probability $\adv$ outputs $x'$ such that $x\neq x'$ and $F(x)=F(x')$ is negligible in $\lambda$.
    \end{enumerate}
\end{definition}

\subsubsection{Construction.}

We are now ready to construct a family of PD-UOWHFs from any PD-OWFs. This is done through an application of the Generalization Lemma \ref{lem:gener PRG} on Rompel's construction of UOWHF from any OWF \cite{R90}. The proof can be found in App.~\ref{app:signatures}.
%This will be useful in the construction of digital signatures. 

\begin{theorem}\label{th:uowhfowf}
    Let $m\coloneqq m(\lambda)$ and $\mu\coloneqq \mu(\lambda)$ be polynomials on the security parameter $\lambda$. Assuming the existence of a $\mu$-PD-OWF $f:\{0,1\}^m\rightarrow \{0,1\}^m$, there exists a $({\mu}{m^{21}\log(m)})$-PD-UOWHF family mapping $O(m^{15})$-bits to $O(m^{14})$-bits.\louis{this is a bit weird, from $O(m^{15})$ bits to $O(m^{14})$ bits
    is not necessarily a hashing function!}
\end{theorem}









\begin{comment}
\section{Multi-sample secure Bot-PD-PRG from short output PRS}
\amit{Need to change the section}

\begin{definition}
    \begin{align}
        &| \Pr \left[ A_{\secpar}(y_1,\ldots,y_q) = 1 :k\xleftarrow{\$} \{0,1\}^\secpar, y_1,\ldots,y_q \gets (G(k))^{\tensor q} \right]\\
        &- \Pr\limits_{y \gets \{0,1\}^{\ell(\secpar)}} \left[ A_{\secpar}(z_1,\ldots,z_q) = 1 :\xleftarrow{\$} \{0,1\}^\secpar, y_1,\ldots,y_q \gets (G(k))^{\tensor q}, z_i=\isbot(y_i,y)\forall i\in [q]\right] |\\
        &\leq \epsilon(\secpar).\label{eq:multi-sample-pseudorandomness-prg}
    \end{align}
    where $\isbot(a,b)$ outputs $\bot$ if $a=\bot$, else outputs $b$. %the probability of the first experiment is over the the randomness of $\keygen$, $G$ and  $A$.\[dd\]
\end{definition}

\amit{
Construction and proof sketch.

\begin{enumerate}
    \item Construction: The same construction, i.e., we first use the extractor on the pseudorandom state and then repeat this process many times to do a bot check, succeeding which we do a majority vote to get a syntactically bot-\pdprg, and then do the XOR repetitions ($\theta(\secpar)$ suffices), wherein the XOR outputs $\bot$ if any of the input is a bot. We can show that despite the XOR repetitions, pseudodeterminism for a random key is $1-\frac{1}{\poly}$, and for every seed $k$, there exists a string $y_k$ except with negligible probability, the output is in $\{y_k,\bot\}$.
    \item Proof: First, invoke the pseudorandomness property to switch to the Haar random states.
    \item Use the property of the extractor to prove that conditioned on the state being in the good set, the distinguishing probability is at most $O(d(\secpar)^{-\frac{1}{6}})$. This is because the good set has $1-\negl$ pseudodeterminisim, and hence, except with negligible probability, the $q$-samples would be all equal, and therefore the distinguishing probability is at most the single copy indistinguishability conditioned on the state being in the good set. The number of repetitions would be roughly a constant times what is done in~\cite{ALY23}.%, and hence the drop in pseudodeterminism is the same as that we will get by doing the bot construction on their $\pdprg$, upto an arbitrarily small constant factor. 
    \amit{I do not know if we need to determine Pseudodeterminism in the sense of the number of keys that have large probability of never outputting bot.}
    \item Furthermore, by the extractor property, the state sampled would be in the good set except with $O(d(\secpar)^{-\frac{1}{6}})$ probability.
    \item Therefore the total distinguishing probability in \cref{eq:multi-sample-pseudorandomness-prg} is at most $O(d(\secpar)^{-\frac{1}{6}})$ which is a fixed inverse polynomial independent of $q$. Hence we can do amplification by the XOR lemma with the same parameters as done in~\cite{ALY23} (upto a $1+\frac{1}{poly}$), to achieve the same negligible pseudorandomness while maintaining the same stretch.
    \item Doing the XOR lemma on output strings that include bot, might be challenging. One way to deal with it is to treat $\bot$ as a special symbol such that if any of the input is $\bot$, the XOR or the $\oplus$ operation outputs $\bot$ else, the $\oplus$ operation works as usual. Note that this way can again ensure the output of the XOR of $\alpha$-parallel and independent folds is either $\bot$ or a fixed value. Note that if the state is in the good set we never will see $\bot$ except with negligible probability, and conditioned in the good set the pseudorandomness holds up to $O(d(\secpar)^{-\frac{1}{6}})$ error. Hence, if we do the XOR operation for $\alpha$ many repetitions, then the conditioned in the good set, the pseudorandomness error will be negligible where $\alpha$ is the same as the number of repetitions made in~\cite{ALY23}. However, if the sample only $\alpha$ independent states, the probability that all of them will be in the good set would be small. Therefore, we will sample $\alpha'=\alpha/(1-q')$ where $q'$ is such that the fraction of bad states is smaller than $q'$ by an inverse polynomial while ensuring $\alpha'=\alpha(1-q')\secpar<\secpar^d(\secpar)^{1/6}=\secpar^{c/6}$, to maintain the stretch. This way, by Chernoff bound, except with negligible probability, the number of states out of the $\alpha'$ states that are in the good set is at least $\alpha$. Note that if at least $\alpha$ of the keys are good, then their $\oplus$ will be negligibly close to uniformly random by the XOR lemma, and hence the overall output conditioned on not being bot will be negligibly close to uniformly random. Combining the last two sentences, we conclude pseudorandomness.
    Next, we need to make sure the stretch is the same or similar to that in~\cite{ALY23}.
    In~\cite{ALY23}, we saw that the key length $\alpha \secpar$ is asymptotically smaller than $\secpar^{c/6}$, the output length. Hence, for any constant $g>1$, it must be the case that the key length in our construction $\alpha'=\alpha(1-q')\secpar< g\alpha\secpar$ is also as asymptotically smaller than $\secpar^{c/6}$, thus maintaining the same multiplicative stretch as~\cite{ALY23} up to a constant (can be made as close as we need to $1$) loss.
\end{enumerate}
}
\end{comment}
% \anote{Add the definition of the parallel version and then remove $q$.}
% \begin{theorem}\label{thm:parallel-repetition-multi-sample-bot-pseudorandomness}
%     A $\pdprg$ with recognizable abort that satisfies multi-sample $\bot$ pseudorandomness, also satisfies the $q$-fold parallel version of multi-sample $\bot$ pseudorandomness for $q\in \poly$.
% \end{theorem}

% \begin{proof}
%     Standard hybrid arguments for parallel repetition of single-round games. 
% \end{proof}

% \input{Bot-PRF-from-Bot-PRG}







%Bib-repetition
@article{GGH16,
  title={Candidate indistinguishability obfuscation and functional encryption for all circuits},
  author={Garg, Sanjam and Gentry, Craig and Halevi, Shai and Raykova, Mariana and Sahai, Amit and Waters, Brent},
  journal={SIAM Journal on Computing},
  volume={45},
  number={3},
  pages={882--929},
  year={2016},
  publisher={SIAM}
}

@misc{NC02,
  title={Quantum computation and quantum information},
  author={Nielsen, Michael A and Chuang, Isaac},
  year={2002},
  publisher={American Association of Physics Teachers}
}




\subsection{Proof of \cref{thm:uowhf}}
\label{app:uowhf}
\begin{proof}
We first describe the construction from traditional $\PRG$s to show that the $\PRG$  is only invoked on uniformly random inputs. This then allows us to apply Generalization \cref{lem:gener PRG} in order to deduce that security holds if we instead use a $\PDPRG$. 

First of all, it is well known that a $\PRG$ $G:\{0,1\}^\ell \rightarrow \{0,1\}^m$ can be converted into a OWF in the following way. Define the function $f: \{0,1\}^{m}\rightarrow \{0,1\}^{m}$ by $f(z)=f(x,y)\coloneqq G(x)$ where the input $z\in \{0,1\}^{m}$ is parsed into $x\in \{0,1\}^{\ell} $ and $y\in \{0,1\}^{m-\ell}$. %It is clear that $f$ satisfies the pseudo-determinism condition for PD-OWFs (Definition \ref{def:PD-OWF}). 

Rompel \cite{R90} showed how to construct UOWHF from any OWF. Let $l(m)\coloneqq \lceil \log(m) \rceil$, $k(m)\coloneqq 2^{l(m)}$ and $n(m)\coloneqq m+4k(m)+l(m)+2$.  

We first construct the function $f_0:\{0,1\}^n\rightarrow \{0,1\}^n$ as follows:
\begin{align*}
    f_0(x,y,i)\coloneqq (f(x),(y\wedge (1^i0^{4k(m)-i}),i))
\end{align*}
where $\wedge$ is bitwise AND.

Next, randomly choose $h_1$ from a $n$-universal family of hash functions mapping $\{0,1\}^{n/2+\log(n)}\rightarrow \{0,1\}^n$ and randomly choose $h_2$ from a $n$-universal family of hash functions mapping $\{0,1\}^{n}\rightarrow \{0,1\}^{(n/2-2\log(n))}$. Define: 
\begin{align*}
    f_1(x)\coloneqq h_2(f_0(h_1(x))).
\end{align*}

Let $f_2:\{0,1\}^{n^6+2n^5\log(n)}\rightarrow \{0,1\}^{n^6-4n^5\log(n)}$ be the function which runs $2n^5$ copies of $f_1$ with independently chosen functions $h_1^i$ and $h_2^i$ for each. In particular, sample $h_1^i$ and $h_2^i$ randomly for $i\in \{1,\ldots,2n^5\}$ and define:
\begin{align*}
    f_2(x^1,\ldots,x^{2n^5})\coloneqq  (f_1^{1}(x^1),\ldots,f_1^{2n^5}(x^{2n^5})).
\end{align*}
where $f_1^i(x)\coloneqq h^i_2(f_0(h^i_1(x)))$.

Let $l\in \mathbb{N}$. Randomly choose $h_3$ from a $2$-universal family of hash functions mapping $\{0,1\}^{n^6+2n^5\log(n)-l}\rightarrow \{0,1\}^{n^6+2n^5\log(n)}$. Define:
\begin{align*}
    f_{3,l}(x)\coloneqq f_2(h_3(x)).
\end{align*}
Randomly sample hash function $h_4$ mapping $\{0,1\}^{n^6-4n^5\log(n)}$ to $ \{0,1\}^{n^6+2n^5\log(n)-l-n/50}$ and define:
\begin{align*}
    f_{4,l}(x)\coloneqq h_4(f_{3,l}(x)).
\end{align*}
Now we achieved a compression by a factor of at least $1-\frac{1}{50n^5}$. Hence, if we start with $O(n^8)$ copies in parallel, we can compress by a factor of $O(n^3)$. Let $f_{5,l}$ be this parallel computation. Finally, let $f_6(x)$ output $f_{5,l}(x)$ for $O(n^2)$ specific values $l$ (see \cite{R90} for more details).  

To summarize, a $\PRG$  can be converted into a OWF $f$, and $f$ can be converted into a UOWHF $f_6$ hashing with a factor of $n$. 

Now assume we instead base the construction on a $(\mu,\ell,m)$-$\PDPRG$ $\tilde{G}$ and let $\tilde{f},\tilde{f}_1,\ldots, \tilde{f}_6$ be the resulting functions. Note that the different choices of hash functions used throughout give a class which we denote by $\mathcal{H}_6$. Our goal is to show that $\mathcal{H}_6$ acts as a $\PDOWHF$ family. We first show the pseudo-determinism property. Let $p\in  O(n^{15})$ indicate the input length for $\tilde{f}_6$. 

\begin{claim}
$\mathcal{H}_6$ satisfies pseudodeterminism condition of ${\mu}{m^{20}\log(m)}$-$\PDOWHF$. 
\end{claim}

\begin{proof}
We first calculate how many evaluations of $\tilde{G}$ are used in one evaluation of $\tilde{f}_6$. Note that $f$ calls $\tilde{G}$ once, $\tilde{f}_1$ calls $\tilde{f}$ once, $\tilde{f}_2$ calls $\tilde{f}_1$ $2n^5$ times, $\tilde{f}_3$ calls $\tilde{f}_2$ once, $\tilde{f}_4$ calls $\tilde{f}_3$ once, $\tilde{f}_{5,l}$ calls $\tilde{f}_{4,l}$ $O(n^{13}\log(n))$ times, and $\tilde{f}_6$ calls $\tilde{f}_{5,l}$ $O(n^2)$ times, giving a total of $O(n^{20}\log(n))=O(m^{20}\log(m))$ calls to $\tilde{G}$ throughout a single evaluation of $\tilde{f}_6$. 
    
Let $x$ be chosen independent of the choice of $\tilde{f}_6$ from the class $\mathcal{H}_6$. Note that that the first computation on $x$ is to evaluate it with a hash function $h_3$ chosen randomly from a 2-universal class of hash functions. Hence, the output of this computation is uniformly distributed given $x$ is chosen independent of $h_3$. Furthermore, applying other hash functions on the result maintains this uniform distribution by the same reasoning. 

In particular, as long as the input is chosen independent of $\tilde{f}_6$, then the computation consists of $O(m^{20}\log(m))$ computations of $\tilde{G}$ on uniformly sampled inputs. Hence, the probability that all these evaluations are in the good set of $\tilde{G}$ is 
    \[(1-{\mu})^{m^{20}\log(m)}\geq  1-{m^{20}\log(m)}{\mu}.\] 

    In the case where all the inputs are in the good set, then the most likely output of $\tilde{f}_6(x)$ corresponds to the most likely output of all the evaluations of $\tilde{G}$. It is easy to show that the probability of obtaining the most likely output is also at least $1-{m^{20}\log(m)}{\mu}$. Hence, $\tilde{f}_6$ satisfies pseudodeterminism condition with parameter ${\mu}{m^{20}\log(m)}$.
    \qed
\end{proof}

\begin{claim}
    $\mathcal{H}_6$ satisfies the security conditions of $\PDOWHF$. 
\end{claim}

\begin{proof}
    To show security for $\PDOWHF$, there are two requirements that need to be met:
    \begin{enumerate}
        \item (One-wayness) For any $\tilde{f}_6\in \mathcal{H}_6$ and QPT inverter $\adv$:
        \begin{align*}
             \Pr_{x\leftarrow \{0,1\}^p}[\tilde{f}_6(\adv(\tilde{f}_6(x)))=\tilde{f}_6(x)]\leq \negl[\lambda].
        \end{align*}

        \item (Collision-resistance) For every QPT algorithm $\adv$, if $\adv$ outputs $x$ and then is given $\tilde{f}_6\leftarrow \mathcal{H}_6$, then the probability $\adv$ outputs $x'$ such that $x\neq x'$ and $\tilde{f}_6(x)=\tilde{f}_6(x')$ is negligible in $\lambda$.
    \end{enumerate}

In the first requirement, $\tilde{f}_6$ is evaluated on a uniformly random input. In the second requirement, it is evaluated on an input chosen independently of the choice of $\tilde{f}_6$ in $\mathcal{H}_6$. By the same arguments used earlier, this implies both security experiments evaluate $\tilde{G}$ on uniformly random values. Hence, the Generalization \cref{lem:gener PRG} implies that both security requirements are satisfied.
\qed
\end{proof}
Hence, the class $\mathcal{H}_6$ satisfies all requirements for ${\mu}{m^{20}\log(m)}$-$\PDOWHF$. 
\qed
\end{proof}


\input{proof_bot_prg_from_pdprg}




















\subsection{One-Time Signatures}
\label{sec:sig 1}
As an application to $\botUOWHF$, we can construct a one-time signature scheme with classical signatures and keys similarly to Lamport's one-time signature scheme \cite{L79}. 

\begin{construct}
    \label{con:one-time sig}
    Let $w\coloneqq w(\lambda)$, $n\coloneqq n(\lambda)$ $\mu\coloneqq \mu(\lambda)$, $q\coloneqq q(\lambda)$, and $\ell\coloneqq \ell(\lambda)$ be polynomials on the security parameter $\lambda$ such that $q(\lambda) >w(\lambda)$ and $n(\lambda)>\lambda$. Let $\mathcal{H}_{\lambda}$ be a $(\mu,\ell,q/w,w)$-$\botUOWHF$ family where $\mu<\frac{1}{2w+1}$. Set $n\coloneqq 2\mu^2$. The construction for a one-time signature scheme on $q$-bit messages is as follows:
    \begin{itemize}
        \item $\textsf{KeyGen}(1^\lambda):$ 
        \begin{enumerate}
            \item Sample $k_i\gets \{0,1\}^\ell$ and $r_i\gets \{0,1\}^q$ for each $i\in [n]$.
            \item Set $F_i(\cdot)=\mathcal{H}_\lambda(k_i,\cdot)$.
            \item For each $i\in [n]$, $j\in [w]$, and $b\in \{0,1\}:$
            \begin{enumerate}
                \item Sample $x_{i,j,b}\gets \{0,1\}^{q}$.
                \item Sample $y_{i,j,b}\gets F_i(x_{i,j,b})$
            \end{enumerate}
            \item Set $\sk\coloneqq (x_{i,j,b})_{i\in [n],j\in [w],b\in \{0,1\}}$ and $\vk\coloneqq (k_i,r_i, y_{i,j,b})_{i\in [n],j\in [w],b\in \{0,1\}}$.
            \item Output $(\sk,\vk)$.
        \end{enumerate}   

        \item $\textsf{Sign}(\sk,m):$ 
        \begin{enumerate}
            \item Compute $m^i\gets F_i(m\oplus r_i)$ for each $i\in [n]$.
            \item Output $\sigma \coloneqq (x_{i,j,m^i_j})_{i\in [n],j\in [w]}$ (interpret $x_{i,j,\bot_j}$ as $\bot$). 
        \end{enumerate}
        
        \item $\textsf{Verify}(\vk,m,\sigma):$ 
        \begin{enumerate}
            \item Interpret $\sigma$ as $(x_{i,j})_{i\in [n],j\in [w]}$ and $\vk$ as $(k_i,r_i,y_{i,j,b})_{i\in [n],j\in [w],b\in \{0,1\}}$.
            \item Compute $m^i\gets F_i(m\oplus r_i)$ for each $i\in [n]$.
            \item For each $j\in [w]$ and $i\in [n]$, compute $y'_{i,j}\gets F_i(x_{i,j})$ (interpret $F_i(\bot)$ as $\bot$). 
            \item If there exists $i\in [n]$ such that $y'_{i,j}=y_{i,j,m^i_j}\neq \bot$ for all $j\in [w]$, then output $\top$.
            \item Otherwise, output $\perp $.
        \end{enumerate} 
    \end{itemize}
\end{construct}

\begin{lemma}[Correctness]\label{lem:ots corr}
    \cref{con:one-time sig} is a correct one-time signature scheme assuming the existence of $\botUOWHF$. 
\end{lemma}

\begin{proof}
Fix $m\in \{0,1\}^q$ and sample $(\sk,\vk)\gets \textsf{KeyGen}(1^\lambda)$, where $\sk\coloneqq (x_{i,j,b})_{i\in [n],j\in [w],b\in \{0,1\}}$ and $\vk\coloneqq (k_i,r_i, y_{i,j,b})_{i\in [n],j\in [w],b\in \{0,1\}}$. Let $\mathcal{G}_i$ denote the good set of inputs for $F_i$. 

For any $i\in [n]$, the probability that $(x_{i,j,b})_{j,b}\subset \mathcal{G}$ and $(m\oplus r_i)\in \mathcal{G} $ is at least $p\coloneqq (1-\mu)^{2w+1}\geq \frac{1}{4}$ by the pseudodeterminism of $F$ and $\mu<\frac{1}{2w+1}$. Hence, the probability that none of the $i\in [n]$ satisfy this condition is $(1-p)^n\leq \negl[\lambda].$

If there exists an $i\in [n]$ such that this condition is satisfied, then it is easy to see that by the pseudodeterminism property of $F$, the verification algorithm will output $\top$ except with negligible probability. 
\qed
\end{proof}

\begin{lemma}[Security]
\label{lem:ots}
\cref{con:one-time sig} is SUF one-time signature scheme assuming the existence of $\botUOWHF$. 
\end{lemma}

\begin{proof}[sketch]
It is clear by the security of $\botUOWHF$, that any QPT adversary cannot find an inverse to any non-$\perp$ image. Moreover, even given a preimage, no QPT adversary can find a different preimage by the collision-resistance property of $\botUOWHF$.   
    \qed
\end{proof}

Henceforth, we denote a one-time signature scheme on $\ell$-bit messages, with verification key length $p$, and where the key generation algorithm makes $q$ coin tosses as a $(\ell,p,q)$-OTS. 

%Note that in \cref{con:one-time sig}, the length of the verification key is $2\cdot n\cdot w=4\cdot \mu^2 \cdot w$. In the next section, we will need to sign a messages consisting of concatenation of two verification keys. Hence, we will need $\ell\geq 8\times \mu^2 \times w$. 

\subsection{One-Time Signatures}
\label{sec:sig 1}
As an application to $\botUOWHF$, we can construct a one-time signature scheme with classical signatures and keys similarly to Lamport's one-time signature scheme \cite{L79}. 

Traditionally, one-time SUF requires that an adversary that receives a signature of a message of its choice, cannot forge a new valid message-signature pair. However, in our case, the signing algorithm may be non-deterministic, hence we need to guarantee SUF against an adversary that receives multiple signatures of a single message of its choice. We call this experiment one-message SUF.

\smallskip \noindent\fbox{%
    \parbox{\textwidth}{%
\textbf{Experiment} $\textsf{Sign}^{\text{OM-SUF}}_{\Pi, \adv}({\lambda})$:
\begin{enumerate}
    \item Sample $(\sk,\vk)\leftarrow \textsf{Gen}(1^\lambda)$.
    \item $\adv$ is given $\vk$ and classical access to the signing oracle $\textsf{Sign}(\sk, \cdot)$.
    \item Let $\mathcal{Q}$ denote the set of messages-signature pairs returned by the signing oracle.
    \item $\adv$ outputs a forgery $(m^*,\sigma^*).$
   \item The output of the experiment is $1$ if:
   \begin{enumerate}
       \item All of the queries were on the same message.
       \item $ (m^*,\sigma^*)\notin \mathcal{Q}$.
       \item $\textsf{Verify}(\vk, m^*, \sigma^*)=1$.
   \end{enumerate}
   \item Otherwise, the output is 0. 
\end{enumerate}}}
\smallskip

\begin{definition}
    A signature scheme $\Pi$ is \emph{one-message strongly unforgeable ({OM-SUF})}, if for any QPT $\adv$,
    \begin{align*} 
        \Pr [\textsf{Sign}^{\textit{OM-SUF}}_{\Pi, \adv}({\lambda})=1]\leq \negl[\lambda].
    \end{align*}
\end{definition}

We now provide a construction for a signature scheme satisfying OM-SUF using $\botUOWHF$. In our scheme, there is a non-negligible probability that verification of a valid signature fails, however, we will later achieve correctness in the final signature scheme (Construction \ref{con:correct sig}).

\begin{construct}
    \label{con:one-time sig}
    Let $\lambda\in \mathbb{N}$ be the security parameter. Let $q$ be polynomial in $\lambda$ and let $w\coloneqq q/\lambda$. Let $\mu= O(1/(3w+4)^2)$. Let $\mathcal{H}_{\lambda}$, $\mathcal{H}'_{\lambda}$, and $\mathcal{H}''_{\lambda}$ be $\botUOWHF$ families with parameters $(\mu,\ell,2,\lambda/2)$, $(\mu,\ell',(q/2+\ell'')/w,w)$, and $(\mu,\ell'',2,q/2)$, respectively, for some polynomials $\ell,\ell',\ell''$ in $\lambda$. The construction for a one-time signature scheme on $q$-bit messages is as follows:
    \begin{itemize}
        \item $\textsf{KeyGen}(1^\lambda):$ 
        \begin{enumerate}
            \item Sample $k\gets \{0,1\}^\ell$ and $k'\gets \{0,1\}^{\ell'}$.
            \item Let $F(\cdot)$ and $F'(\cdot)$ denote $\mathcal{H}_\lambda(k,\cdot)$ and $\mathcal{H}'_\lambda(k',\cdot)$, respectively.
            \item For each $j\in [w]$, and $b\in \{0,1\}:$
            \begin{enumerate}
                \item Sample $x_{j,b}\gets \{0,1\}^{q}$.
                \item Sample $y_{j,b}\gets F(x_{j,b})$
            \end{enumerate}
            \item Set $\sk\coloneqq (x_{j,b})_{j\in [w],b\in \{0,1\}}$ and $\vk\coloneqq (k,k', y_{j,b})_{j\in [w],b\in \{0,1\}}$.
            \item Output $(\sk,\vk)$.
        \end{enumerate}   

        \item $\textsf{Sign}(\sk,m):$ 
        \begin{enumerate}
        \item Sample $k''\gets \{0,1\}^{\ell''}$ and set $F''(\cdot)$ as $H''(k'',\cdot)$.
            \item Compute $m'\gets F'(F''(m)\| k'')$\footnote{Here $s\|r$ represents the concatenation of the two strings $s$ and $r$.}.
            \item If $m'=\bot$, then output $\bot$.
            \item Otherwise, output $\sigma \coloneqq (k'',x_{j,m'_j})_{j\in [w]}$. 
        \end{enumerate}
        
        \item $\textsf{Verify}(\vk,m,\sigma):$ 
        \begin{enumerate}
        \item If $\sigma =\bot$, then output $\bot$.
            \item Otherwise, interpret $\sigma$ as $(k'',x_{j})_{j\in [w]}$ and $\vk$ as $(k,k',y_{j,b})_{j\in [w],b\in \{0,1\}}$.
            \item Compute $m'\gets F'(F''(m)\|k'')$. If the result is $\bot$, then output $\bot$. 
            \item For each $j\in [w]$, compute $\tilde{y}_{j}\gets F(x_{j})$. 
            \item If $\tilde{y}_{j}=y_{j,m_j}\neq \bot$ for all $j\in [w]$, then output $\top$.
            \item Otherwise, output $\perp $.
        \end{enumerate} 
    \end{itemize}
\end{construct}

\begin{lemma}[Correctness]\label{lem:ots corr}
    \cref{con:one-time sig} is $(1-\mu)^{3w+4}$-correct one-time signature scheme on $q$-bit messages assuming the existence of $\botUOWHF$s. 
\end{lemma}

\begin{proof}
Fix $m\in \{0,1\}^q$ and sample $(\sk,\vk)\gets \textsf{KeyGen}(1^\lambda)$, where $\sk\coloneqq (x_{j,b})_{j\in [w],b\in \{0,1\}}$ and $\vk\coloneqq (k, y_{j,b})_{j\in [w],b\in \{0,1\}}$. Let the signature of $m$ generated be $\sigma \coloneqq (k'',x_{j,m'_j})_{j\in [w]}$. Let $\mathcal{G}$, $\mathcal{G}'$, and $\mathcal{G}''$ denote the good set of inputs for $F$, $F'$ and $F''$. 

By the pseudodeterminism of $\botUOWHF$s, the probability that $(x_{j,b})_{j,b}\subset \mathcal{G}$, $F''(m)\|k'' \in \mathcal{G}' $ and $m\in \mathcal{G}''$ is at least $p\coloneqq (1-\mu)^{2w+2}$. In this case, it is easy to check that the verification algorithm will output $\top$ if all $w+2$ evaluations performed return the most likely output. There exists a negligible function $\negl[\lambda]$ such that for an input in these good sets, the evaluation will yield the most likely output except with $\negl[\lambda]$ probability. To sum up, all these events together occur with probability $p(1- \negl[\lambda])^{w+2}\geq (1-\mu)^{3w+4}$.
\qed
\end{proof}

\begin{lemma}[Security]
\label{lem:ots}
If $\mu= O(1/(3w+4)^2)$, then \cref{con:one-time sig} is OM-SUF signature scheme on $q$-bit messages assuming the existence of $\botUOWHF$s. 
\end{lemma}

\begin{proof}[sketch]
Assume there exists a QPT algorithm $\adv$ such that $\Pr [\textsf{Sign}^{\textit{OM-SUF}}_{\Pi, \adv}({\lambda})=1]$ is non-negligible. We will construct a QPT algorithm $\mathcal{B}$ that breaks the collision-resistance of one of the $\botUOWHF$s used in the construction. 

%Recall, in the collision-resistance security experiment, the adversary first outputs an input $x$ and then receives a hash function $F$ sampled from the family of $\botUOWHF$, and needs to try and return a collision $x'$ such that $H(x)=H(x')$. 

The algorithm of $\mathcal{B}$ is as follows:

\begin{enumerate}
    \item For each $j\in [w]$, and $b\in \{0,1\}$, sample $x_{j,b}\gets \{0,1\}^{q}$.
    \item Receive a challenge key $k\gets \{0,1\}^\ell$ from the experiment. 
    \item For each $j\in [w]$, and $b\in \{0,1\}$, sample $y_{j,b}\gets F(k,x_{j,b})$.
    \item Receive a challenge key $k'\gets \{0,1\}^{\ell'}$ from the experiment. 
    \item Set $\sk\coloneqq (x_{j,b})_{j\in [w],b\in \{0,1\}}$ and $\vk\coloneqq (k,k', y_{j,b})_{j\in [w],b\in \{0,1\}}$.
 \item Give $\adv$ the key $\vk$ and classical access to the signing oracle $\textsf{Sign}(\sk, \cdot)$.
    \item $\adv$ outputs a forgery $(m^*,\sigma^*)$. Interpret $\sigma^*$ as $(k'',x'_{j})_{j\in [w]}$.
    \item $\mathcal{B}$ checks:   
    \begin{enumerate}
       \item All of the queries were on the same message, say $m$.
       \item $ (m^*,\sigma^*)\notin \mathcal{Q}$.
       \item $\textsf{Verify}(\vk, m^*, \sigma^*)=1$.
   \end{enumerate}
   \item If one of the conditions is not satisfied, then output $\bot$.
   \item Check if one of the following conditions is satisfied:
   \begin{enumerate}
       \item If for some $j\in [w]$, $x_j\neq x_j'$ and $F(k,x_j)=F(k,x_j')$, $\mathcal{B}$ outputs $(x_j,x_j')$.
       \item If for some $\tilde{k}$ in a signature in $\mathcal{Q}$, $F(k',m^*)\|k'\neq F(\tilde{k},m)\|\tilde{k}$ and $F(k,F(k',m^*)\|k')=F(k,F(\tilde{k},m)\|\tilde{k})$, then $\mathcal{B}$ outputs $(F(k',m^*)\|k', F(\tilde{k},m)\|\tilde{k})$.
       \item If for some $\tilde{k}$ in a signature in $\mathcal{Q}$, $F(k',m^*)\|k'= F(\tilde{k},m)\|\tilde{k}$ and $m\neq m^*$, then $\mathcal{B}$ outputs $(m,m^*)$.
   \end{enumerate} 
   \item Otherwise, output $\perp$. 
\end{enumerate}

It is easy to check that if Step 11 is passed, then one of the conditions in Step 13 will be satisfied with high probability. In which case, $\mathcal{B}$ succeeds in finding a collision for a hash function on an input that is distributed uniformly and independently of the function. Note that Step 11 is passed with non-negligible probability given that $\Pr [\textsf{Sign}^{\textit{OM-SUF}}_{\Pi, \adv}({\lambda})=1]$ is non-negligible.  
    \qed
\end{proof}

%Note that in \cref{con:one-time sig}, the length of the verification key is $2\cdot n\cdot w=4\cdot \mu^2 \cdot w$. In the next section, we will need to sign a messages consisting of concatenation of two verification keys. Hence, we will need $\ell\geq 8\times \mu^2 \times w$. 


\ifnum\iacr=1
\section{Digital Signatures (Overview)}
In this section, we discuss how we construct digital signatures from $\SPRS$ using our tools of $\botUOWHF$s and $\botPRF$. This is done in several steps and we only give an outline in the main paper and refer the reader to \cref{sec:Sig} for details. 

First of all, we define strong unforgeability for deterministic one-time signatures in the non-deterministic setting yielding \emph{one-message signatures (OMS)}. This allows an adversary to receive multiple signatures for the same message. Then, we build OMSs that enable signing long messages using $\botUOWHF$s based on the approach in the classical case given in Section 6.5.2 of \cite{Gol04}. This is important since we will need to sign messages that are double the length of the verification key in order to build many-message signatures. 

Then, we enable signing many messages but where the signer needs to store previous signatures following the approach given in \cite{NY89} with minimal modifications. The signer needs to store previous signatures so this approach is called \emph{stateful}. 

Finally, we upgrade our construction to a stateless digital signature scheme using our construction for $\botPRF$s following a similar approach to \cite{Gol04}, which is based on traditional $\PRF$s. 

A problem with our approach is that our reliance on pseudodeterministic function only yields a signature scheme with inverse-polynomial correctness. We can improve correctness, reducing the error to a negligible value, through repetition by generating multiple signatures. However, the resulting scheme is no longer strongly unforgeable since an adversary that receives two correct signatures in the repeated scheme can output only one of the signatures and replace the rest with $\bot$ to generate a new signature. Nevertheless, our results give the option to choose between statistical correctness and strong unforgeability.


\begin{theorem}[Digital signatures from $\SPRS$]
    Let $\lambda \in \mathbb{N}$ be the security parameter. Assuming the existence of $c\log(\lambda)$-$\PRS$ with large enough $c\in \mathbb{N}$, there exists stateless (many-message) digital signatures on $\lambda$-bit messages with classical keys satisfying UF as well as statistical correctness. 
\end{theorem}



\fi
